Dipole-dipole interactions mediated by a photonic flat band

Flat bands (FBs) are energy bands with zero group velocity, which in electronic systems were shown to favor strongly correlated phenomena. Indeed, a FB can be spanned with a basis of strictly localized states, the so called "compact localized states" (CLSs), which are yet generally non-orthogonal. Here, we study emergent dipole-dipole interactions between emitters dispersively coupled to the photonic analogue of a FB, a setup within reach in state-of the-art experimental platforms. We show that the strength of such photon-mediated interactions decays exponentially with distance with a characteristic localization length which, unlike typical behaviours with standard bands, saturates to a finite value as the emitter's energy approaches the FB. Remarkably, we find that the localization length grows with the overlap between CLSs according to an analytically-derived universal scaling law valid for a large class of FBs both in 1D and 2D. Using giant atoms (non-local atom-field coupling) allows to tailor interaction potentials having the same shape of a CLS or a superposition of a few of these.

==> old/section01.tex <==
\section{Introduction} 
\label{sec:introduction}

\textit{Flat Bands} (FBs) are a special type of energy bands, which can occur in natural and artificial lattices \cite{doi:10.1080/23746149.2021.1878057, doi:10.1080/23746149.2018.1473052,Xia:16}. Unlike standard bands, FBs are \textit{dispersionless}, \ie particles occupying such a band have \textit{zero} velocity at any wavelength. 
For this reason, photonic FB systems have been studied to achieve exotic regimes of light localization \cite{TangSongXiaXiaMaYanHuXuLeykamChen+2020+1161+1176}. 
Remarkably, FBs have a macroscopically large degeneracy, even diverging in the thermodynamical limit, making them extremely sensitive to small perturbations, like disorder \cite{PhysRevB.88.224203} and nonlinearities \cite{10.1038/s41598-020-62079-8}. This renders FB systems an intriguing platform to explore highly-correlated phases of matter \cite{10.1038/s42005-023-01292-z}.

Owing to the degeneracy of the FB energy, it has been shown \cite{PhysRevB.99.045107} that the FB eigenspace can be spanned by eigenstates which are localised on a vanishing fraction of the bath, in a way reminiscent of Wannier orbitals in solid-state systems \cite{PhysRevB.95.115309}. These states are dubbed \textit{Compact Localised States} (CLSs) and, in the most general case, form a non-orthogonal basis of the FB eigenspace.
CLSs have been observed in several photonic platforms \cite{loc_Lieb1,loc_Lieb2,Zong:16}, as well as in systems based on resonant circuits \cite{chasemayoral2023compact}.

Another interesting feature of FBs emerges in the case of a \textit{band touching}, \ie when one or multiple dispersive bands cross the FB energy. 
In some of these cases (\textit{singular} FBs), a new type of topology emerges, dubbed \textit{real-space topology} \cite{PhysRevB.99.045107} and, as a consequence, a certain number of extended states, named \textit{Non-contraptible Loop States} (NLSs), have to be added in the bulk of the system to the CLSs basis in order to span the FB eigenspace.

In this work, we explore the case of several Quantum Emitters (QEs) coupled to a photonic structured environment having at least a FB in its spectrum.
Indeed, QEs interacting with low-dimensional environments emerged in the last few years as an intriguing platform both for fundamental purposes \cite{doi:10.1126/sciadv.aaw0297, PhysRevResearch.2.023003, PhysRevA.89.053826,RevModPhys.95.015002} and technological applications \cite{PhysRevLett.131.073602}. 
In particular, it has been shown that, under the weak-coupling approximation, QEs in the dispersive regime might be used as a tool for simulating specific quantum spin Hamiltonian \cite{douglas-chang}, whose parameters depend on the features of the atom-photon bound states (BSs) \cite{DressedLuca2021} formed by each QE.
Nowadays, a richer phenomenology is accessible through the paradigm of \textit{giant} emitters \cite{PhysRevA.107.013710}, each coupling to the bath at multiple distinct points. 
Such emitters show a plethora of new phenomena, unachievable in the small-emitter limit, like frequency-dependent relaxation rates \cite{PhysRevA.90.013837}
and the possibility to engineer decoherence-free Hamiltonians in the photonic continuum \cite{PhysRevResearch.2.043184}.

Surprisingly, in our analysis of QEs coupled to FB systems, we find non-trivial differences in the features of BSs depending on the (non-)orthogonality of the CLSs basis, opening the door to the implementation of finite-ranged spin Hamiltonians through mediated interactions. 
Furthermore, we show that \textit{giant} emitters offer a flexible platform to tailor photon-mediated interactions in a novel way, which does not involve the manipulation of the emitter's frequency \cite{PhysRevA.93.033833}. 

Remarkably, we show that the presence of a FB seeds a new type of localised BS, previously unreported to our knowledge, whose localization length is independent of any frequency of the system.
We name these states as \textit{FB-induced Bound States} (FBBSs).

Regarding time evolution in the single-excitation sector, no difference is found between an atom resonant to a FB and the usual cavity-QED case \cite{Haroche:993568}, owing to the FB dispersionless nature.

Finally, in studying two-dimensional systems in presence of a singular quadratic band touching \footnote{A band touching is said to be \textit{quadratic} if the local expansion of the dispersion law is quadratic around the band touching point.}, we find that a BS is formed even if the emitter is resonant to the band edge of the dispersive band, but no contribution to its shape comes from NLSs in the thermodynamic limit.

% \begin{figure*}[t]
%     \centering
%     \includegraphics{figures/bitmap.png}
%     \caption{(a)}
%     \label{fig:Fig1}
% \end{figure*}
